Fast generation of Schr\"odinger cat states in a Kerr-tunable superconducting resonator

Schr\"odinger cat states, quantum superpositions of macroscopically distinct classical states, are an important resource for quantum communication, quantum metrology and quantum computation. Especially, cat states in a phase space protected against phase-flip errors can be used as a logical qubit. However, cat states, normally generated in three-dimensional cavities, are facing the challenges of scalability and controllability. Here, we present a novel strategy to generate and store cat states in a coplanar superconducting circuit by the fast modulation of Kerr nonlinearity. At the Kerr-free work point, our cat states are passively preserved due to the vanishing Kerr effect. We are able to prepare a 2-component cat state in our chip-based device with a fidelity reaching 89.1% under a 96 ns gate time. Our scheme shows an excellent route to constructing a chip-based bosonic quantum processor.

==> refer_abbr.tex <==
@article{b1,
  title={Quantum supremacy using a programmable superconducting processor},
  author={Arute, Frank and Arya, Kunal and Babbush, Ryan and others},%Bacon, Dave and Bardin, Joseph C and Barends, Rami and Biswas, Rupak and Boixo, Sergio and Brandao, Fernando GSL and Buell, David A and others},
  journal={Nature},
  volume={574},
  number={7779},
  pages={505--510},
  year={2019},
  publisher={Nature Publishing Group}
}
@article{b2,
  title={Fast quantum gates for neutral atoms},
  author={Jaksch, Dieter and Cirac, Juan Ignacio and Zoller, Peter and others},%Rolston, Steve L and C{\^o}t{\'e}, Robin and Lukin, Mikhail D},
  journal={Physical Review Letters},
  volume={85},
  number={10},
  pages={2208},
  year={2000},
  publisher={APS}
}
@article{b3,
  title={Quantum simulations with cold trapped ions},
  author={Johanning, Michael and Var{\'o}n, Andr{\'e}s F and Wunderlich, Christof},
  journal={Journal of Physics B: Atomic, Molecular and Optical Physics},
  volume={42},
  number={15},
  pages={154009},
  year={2009},
  publisher={IOP Publishing}
}
@article{b4,
  title={Josephson persistent-current qubit},
  author={Mooij, JE and Orlando, TP and Levitov, L and others},%Tian, Lin and Van der Wal, Caspar H and Lloyd, Seth},
  journal={Science},
  volume={285},
  number={5430},
  pages={1036--1039},
  year={1999},
  publisher={American Association for the Advancement of Science}
}
@article{b5,
  title={Quantum walks on a programmable two-dimensional 62-qubit superconducting processor},
  author={Gong, Ming and Wang, Shiyu and Zha, Chen and others},%Chen, Ming-Cheng and Huang, He-Liang and Wu, Yulin and Zhu, Qingling and Zhao, Youwei and Li, Shaowei and Guo, Shaojun and others},
  journal={Science},
  volume={372},
  number={6545},
  pages={948--952},
  year={2021},
  publisher={American Association for the Advancement of Science}
}
@article{b6,
  title={Deterministically encoding quantum information using 100-photon Schr{\"o}dinger cat states},
  author={Vlastakis, Brian and Kirchmair, Gerhard and Leghtas, Zaki and others},%Nigg, Simon E and Frunzio, Luigi and Girvin, Steven M and Mirrahimi, Mazyar and Devoret, Michel H and Schoelkopf, Robert J},
  journal={Science},
  volume={342},
  number={6158},
  pages={607--610},
  year={2013},
  publisher={American Association for the Advancement of Science}
}

@article{b7,
  title={Quantum error correction of a qubit encoded in grid states of an oscillator},
  author={Campagne-Ibarcq, Philippe and Eickbusch, Alec and Touzard, Steven and others},%Zalys-Geller, Evan and Frattini, Nicholas E and Sivak, Volodymyr V and Reinhold, Philip and Puri, Shruti and Shankar, Shyam and Schoelkopf, Robert J and others},
  journal={Nature},
  volume={584},
  number={7821},
  pages={368--372},
  year={2020},
  publisher={Nature Publishing Group}
}
@article{b8,
  title={Universal gate set for continuous-variable quantum computation with microwave circuits},
  author={Hillmann, Timo and Quijandr{\'\i}a, Fernando and Johansson, G{\"o}ran and others},%Ferraro, Alessandro and Gasparinetti, Simone and Ferrini, Giulia},
  journal={Physical review letters},
  volume={125},
  number={16},
  pages={160501},
  year={2020},
  publisher={APS}
}
@article{b9,
  title={Propagating Wigner-negative states generated from the steady-state emission of a superconducting qubit},
  author={Lu, Yong and Strandberg, Ingrid and Quijandr{\'\i}a, Fernando and others},%Johansson, G{\"o}ran and Gasparinetti, Simone and Delsing, Per},
  journal={Physical Review Letters},
  volume={126},
  number={25},
  pages={253602},
  year={2021},
  publisher={APS}
}
@article{b10,
  title={Sufficient conditions for efficient classical simulation of quantum optics},
  author={Rahimi-Keshari, Saleh and Ralph, Timothy C and Caves, Carlton M},
  journal={Physical Review X},
  volume={6},
  number={2},
  pages={021039},
  year={2016},
  publisher={APS}
}
@article{b11,
  title={Error-transparent operations on a logical qubit protected by quantum error correction},
  author={Ma, Yuwei and Xu, Yuan and Mu, Xianghao and others},%Cai, Weizhou and Hu, Ling and Wang, Weiting and Pan, Xiaoxuan and Wang, Haiyan and Song, YP and Zou, C-L and others},
  journal={Nature Physics},
  volume={16},
  number={8},
  pages={827--831},
  year={2020},
  publisher={Nature Publishing Group}
}
@article{b12,
  title={Encoding a qubit in an oscillator},
  author={Gottesman, Daniel and Kitaev, Alexei and Preskill, John},
  journal={Physical Review A},
  volume={64},
  number={1},
  pages={012310},
  year={2001},
  publisher={APS}
}
@article{b13,
  title={Quantum control of bosonic modes with superconducting circuits},
  author={Ma, Wen-Long and Puri, Shruti and Schoelkopf, Robert J and others},%Devoret, Michel H and Girvin, Steven M and Jiang, Liang},
  journal={Science Bulletin},
  volume={66},
  number={17},
  pages={1789--1805},
  year={2021},
  publisher={Elsevier}
}
@article{b14,
  title={Robust preparation of Wigner-negative states with optimized SNAP-displacement sequences},
  author={Kudra, Marina and Kervinen, Mikael and Strandberg, Ingrid and others},%Ahmed, Shahnawaz and Scigliuzzo, Marco and Osman, Amr and Lozano, Daniel P{\'e}rez and Thol{\'e}n, Mats O and Borgani, Riccardo and Haviland, David B and others},
  journal={PRX Quantum},
  volume={3},
  number={3},
  pages={030301},
  year={2022},
  publisher={APS}
}
@article{b15,
  title={Observation of quantum state collapse and revival due to the single-photon Kerr effect},
  author={Kirchmair, Gerhard and Vlastakis, Brian and Leghtas, Zaki and others},%Nigg, Simon E and Paik, Hanhee and Ginossar, Eran and Mirrahimi, Mazyar and Frunzio, Luigi and Girvin, Steven M and Schoelkopf, Robert J},
  journal={Nature},
  volume={495},
  number={7440},
  pages={205--209},
  year={2013},
  publisher={Nature Publishing Group}
}
@article{b16,
  title={Confining the state of light to a quantum manifold by engineered two-photon loss},
  author={Leghtas, Zaki and Touzard, Steven and Pop, Ioan M and others},%Kou, Angela and Vlastakis, Brian and Petrenko, Andrei and Sliwa, Katrina M and Narla, Anirudh and Shankar, Shyam and Hatridge, Michael J and others},
  journal={Science},
  volume={347},
  number={6224},
  pages={853--857},
  year={2015},
  publisher={American Association for the Advancement of Science}
}
@article{b17,
  title={One hundred second bit-flip time in a two-photon dissipative oscillator},
  author={Berdou, C and Murani, A and Reglade, U and others},
  journal={arXiv preprint arXiv:2204.09128},
  year={2022}
}
@article{b18,
  title={Stabilization and operation of a Kerr-cat qubit},
  author={Grimm, Alexander and Frattini, Nicholas E and Puri, Shruti and others},%Mundhada, Shantanu O and Touzard, Steven and Mirrahimi, Mazyar and Girvin, Steven M and Shankar, Shyam and Devoret, Michel H},
  journal={Nature},
  volume={584},
  number={7820},
  pages={205--209},
  year={2020},
  publisher={Nature Publishing Group}
}
@article{b19,
  title={Kerr-free three-wave mixing in superconducting quantum circuits},
  author={Sivak, VV and Frattini, NE and Joshi, VR and others},%Lingenfelter, A and Shankar, S and Devoret, MH},
  journal={Physical Review Applied},
  volume={11},
  number={5},
  pages={054060},
  year={2019},
  publisher={APS}
}
@article{b20,
  title={3-wave mixing Josephson dipole element},
  author={Frattini, NE and Vool, U and Shankar, S and Narla, A and Sliwa, KM and others},%Devoret, MH},
  journal={Applied Physics Letters},
  volume={110},
  number={22},
  pages={222603},
  year={2017},
  publisher={AIP Publishing LLC}
}
@article{b21,
  title={Engineering the quantum states of light in a Kerr-nonlinear resonator by two-photon driving},
  author={Puri, Shruti and Boutin, Samuel and Blais, Alexandre},
  journal={npj Quantum Information},
  volume={3},
  number={1},
  pages={1--7},
  year={2017},
  publisher={Nature Publishing Group}
}
@article{b22,
  title={Synthesizing arbitrary quantum states in a superconducting resonator},
  author={Hofheinz, Max and Wang, H and Ansmann, Markus and others},%Bialczak, Radoslaw C and Lucero, Erik and Neeley, Matthew and O'connell, AD and Sank, Daniel and Wenner, J and Martinis, John M and others},
  journal={Nature},
  volume={459},
  number={7246},
  pages={546--549},
  year={2009},
  publisher={Nature Publishing Group}
}
@article{b23,
  title={Experimental determination of the motional quantum state of a trapped atom},
  author={Leibfried, Dietrich and Meekhof, DM and King, BE and others},%Monroe, CH and Itano, Wayne M and Wineland, David J},
  journal={Physical review letters},
  volume={77},
  number={21},
  pages={4281},
  year={1996},
  publisher={APS}
}
@article{b24,
  title={Engineering fast bias-preserving gates on stabilized cat qubits},
  author={Xu, Qian and Iverson, Joseph K and Brand{\~a}o, Fernando GSL and others},%Jiang, Liang},
  journal={Physical Review Research},
  volume={4},
  number={1},
  pages={013082},
  year={2022},
  publisher={APS}
}
@article{b25,
  title={Fast parametric two-qubit gates with suppressed residual interaction using the second-order nonlinearity of a cubic transmon},
  author={Noguchi, Atsushi and Osada, Alto and Masuda, Shumpei and others},%Kono, Shingo and Heya, Kentaro and Wolski, Samuel Piotr and Takahashi, Hiroki and Sugiyama, Takanori and Lachance-Quirion, Dany and Nakamura, Yasunobu},
  journal={Physical Review A},
  volume={102},
  number={6},
  pages={062408},
  year={2020},
  publisher={APS}
}
@article{b27,
  title={Optimizing the nonlinearity and dissipation of a snail parametric amplifier for dynamic range},
  author={Frattini, NE and Sivak, VV and Lingenfelter, A and others},%Shankar, S and Devoret, MH},
  journal={Physical Review Applied},
  volume={10},
  number={5},
  pages={054020},
  year={2018},
  publisher={APS}
}
@book{b28,
author = {Haroche, Serge and Raimond, J.},
year = {2006},
title = {Exploring the Quantum: Atoms, Cavities, and Photons},
publisher = {Oxford Univ Pr}
}
@article{b29,
  title={Reconstruction of non-classical cavity field states with snapshots of their decoherence},
  author={Deleglise, Samuel and Dotsenko, Igor and Sayrin, Clement and others},%Bernu, Julien and Brune, Michel and Raimond, Jean-Michel and Haroche, Serge},
  journal={Nature},
  volume={455},
  number={7212},
  pages={510--514},
  year={2008},
  publisher={Nature Publishing Group}
}
@article{b30,
  title={Resolving Fock states near the Kerr-free point of a superconducting resonator},
  author={Lu, Yong and Kudra, Marina and Hillmann, Timo and others},
  journal={arXiv preprint arXiv:2210.09718},
  year={2022}
}
@article{b31,
  title={Extending the lifetime of a quantum bit with error correction in superconducting circuits},
  author={Ofek, Nissim and Petrenko, Andrei and Heeres, Reinier and others},%Reinhold, Philip and Leghtas, Zaki and Vlastakis, Brian and Liu, Yehan and Frunzio, Luigi and Girvin, SM and Jiang, Liang and others},
  journal={Nature},
  volume={536},
  number={7617},
  pages={441--445},
  year={2016},
  publisher={Nature Publishing Group}
}
@article{b32,
  title={A Schr{\"o}dinger cat living in two boxes},
  author={Wang, Chen and Gao, Yvonne Y and Reinhold, Philip and others},
  journal={Science},
  volume={352},
  number={6289},
  pages={1087--1091},
  year={2016},
  publisher={American Association for the Advancement of Science}
}
@article{b33,
  title={Macroscopic quantum superpositions by means of single-atom dispersion},
  author={Savage, Craig M and Braunstein, Samuel L and Walls, Daniel F},
  journal={Optics letters},
  volume={15},
  number={11},
  pages={628--630},
  year={1990},
  publisher={Optica Publishing Group}
}
@article{b34,
  title={Engineering the quantum states of light in a Kerr-nonlinear resonator by two-photon driving},
  author={Puri, Shruti and Boutin, Samuel and Blais, Alexandre},
  journal={npj Quantum Information},
  volume={3},
  number={1},
  pages={1--7},
  year={2017},
  publisher={Nature Publishing Group}
}
@article{b36,
  title={Continuous-variable quantum teleportation through lossy channels},
  author={Chizhov, AV and Kn{\"o}ll, L and Welsch, D-G},
  journal={Physical Review A},
  volume={65},
  number={2},
  pages={022310},
  year={2002},
  publisher={APS}
}
@article{b37,
  title={Quantum error correction against photon loss using multicomponent cat states},
  author={Bergmann, Marcel and van Loock, Peter},
  journal={Physical Review A},
  volume={94},
  number={4},
  pages={042332},
  year={2016},
  publisher={APS}
}
@article{b38,
author = {Barends, R and Kelly, J and Megrant, A and others},
year = {2014},
month = {04},
pages = {500-3},
title = {Superconducting quantum circuits at the surface code threshold for fault tolerance},
volume = {508},
journal = {Nature},
doi = {10.1038/nature13171}
}
@article{b39,
author = {Yamaji, T. and Kagami, S. and Yamaguchi, A. and Satoh, T. and Koshino, Kazuki and Goto, H. and Lin, Z. and Nakamura, Y. and Yamamoto, T.},
year = {2022},
month = {02},
pages = {},
title = {Spectroscopic observation of the crossover from a classical Duffing oscillator to a Kerr parametric oscillator},
volume = {105},
journal = {Physical Review A},
doi = {10.1103/PhysRevA.105.023519}
}
@article{b40,
author = {Xue, Hang and Lin, Zhirong and Wenbing, Jiang and Niu, Zhengqi and Liu, Kuang and Peng, Wei and Wang, Zhen},
year = {2021},
month = {03},
pages = {},
title = {Fabrication and characterization of all-Nb lumped-element Josephson parametric amplifiers},
volume = {30},
journal = {Chinese Physics B},
doi = {10.1088/1674-1056/abeee6}
}
@article{b41,
  title={Designing Kerr Interactions for Quantum Information Processing via Counterrotating Terms of Asymmetric Josephson-Junction Loops},
  author={Hillmann, Timo and Quijandr{\'\i}a, Fernando},
  journal={Physical Review Applied},
  volume={17},
  number={6},
  pages={064018},
  year={2022},
  publisher={APS}
}
@article{b42,
  title={Quantum simulators: Architectures and opportunities},
  author={Altman, Ehud and Brown, Kenneth R and Carleo, Giuseppe and  others},
  journal={PRX Quantum},
  volume={2},
  number={1},
  pages={017003},
  year={2021},
  publisher={APS}
}
@book{b43,
  title={Fluctuating nonlinear oscillators: from nanomechanics to quantum superconducting circuits},
  author={Dykman, Mark},
  year={2012},
  publisher={Oxford University Press}
}
@article{b44,
  title={Parity measurement in the strong dispersive regime of circuit quantum acoustodynamics},
  author={von L{\"u}pke, Uwe and Yang, Yu and Bild, Marius and Michaud, Laurent and Fadel, Matteo and Chu, Yiwen},
  journal={Nature Physics},
  pages={1--6},
  year={2022},
  publisher={Nature Publishing Group}
}
@article{b45,
  title={Experimental demonstration of continuous quantum error correction},
  author={Livingston, William P and Blok, Machiel S and Flurin, Emmanuel and Dressel, Justin and Jordan, Andrew N and Siddiqi, Irfan},
  journal={Nature communications},
  volume={13},
  number={1},
  pages={1--7},
  year={2022},
  publisher={Nature Publishing Group}
}
@article{b46,
  title={Generation and manipulation of Schr{\"o}dinger cat states in Rydberg atom arrays},
  author={Omran, Ahmed and Levine, Harry and Keesling, Alexander and Semeghini, Giulia and Wang, Tout T and Ebadi, Sepehr and Bernien, Hannes and Zibrov, Alexander S and Pichler, Hannes and Choi, Soonwon and others},
  journal={Science},
  volume={365},
  number={6453},
  pages={570--574},
  year={2019},
  publisher={American Association for the Advancement of Science}
}

==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}


